EPT-1.5 Technical Report

We announce the release of EPT-1.5, the latest iteration in our Earth Physics Transformer (EPT) family of foundation AI earth system models. EPT-1.5 demonstrates substantial improvements over its predecessor, EPT-1. Built specifically for the European energy industry, EPT-1.5 shows remarkable performance in predicting energy-relevant variables, particularly 10m & 100m wind speed and solar radiation. Especially in wind prediction, it outperforms existing AI weather models like GraphCast, FuXi, and Pangu-Weather, as well as the leading numerical weather model, IFS HRES by the European Centre for Medium-Range Weather Forecasts (ECMWF), setting a new state of the art.

==> preamble.tex <==
\section{Supplementary Material}
\label{section:appendix}

\begin{figure*}[!t]
  \centering
  \begin{minipage}[b]
    \centering
    \includegraphics[width=\linewidth]{images/2m_temperature_prediction.png}
    \caption{2m temperature prediction by EPT-1.5}
    \label{fig:2m_pred}
  \end{minipage}
  \hfill
  \begin{minipage}[b]
    \centering
    \includegraphics[width=\linewidth]{images/msl_prediction.png}
    \caption{Mean sea level pressure prediction by EPT-1.5}
    \label{fig:mslp_pred}
  \end{minipage}

  \vspace{1em}

  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/100u_prediction.png}
    \caption{100m wind speed eastward prediction by EPT-1.5}
    \label{fig:100u_pred}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/z500_prediction.png}
    \caption{Geopotential prediction at 500 hPa by EPT-1.5}
    \label{fig:g500_pred}
  \end{minipage}

  \vspace{1em}

  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/r1000_prediction.png}
    \caption{2m relative humidity prediction by EPT-1.5}
    \label{fig:2r_pred}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/ssrd_prediction.png}
    \caption{Solar radiation prediction by EPT-1.5}
    \label{fig:ssrd_pred}
  \end{minipage}

  \caption{Various weather predictions by EPT-1.5}
  \label{fig:all_predictions}
\end{figure*}
